Towards Universal Performance Modeling for Machine Learning Training on Multi-GPU Platforms

Characterizing and predicting the training performance of modern machine learning (ML) workloads on compute systems with compute and communication spread between CPUs, GPUs, and network devices is not only the key to optimization and planning but also a complex goal to achieve. The primary challenges include the complexity of synchronization and load balancing between CPUs and GPUs, the variance in input data distribution, and the use of different communication devices and topologies (e.g., NVLink, PCIe, network cards) that connect multiple compute devices, coupled with the desire for flexible training configurations. Built on top of our prior work for single-GPU platforms, we address these challenges and enable multi-GPU performance modeling by incorporating (1) data-distribution-aware performance models for embedding table lookup, and (2) data movement prediction of communication collectives, into our upgraded performance modeling pipeline equipped with inter-and intra-rank synchronization for ML workloads trained on multi-GPU platforms. Beyond accurately predicting the per-iteration training time of DLRM models with random configurations with a geomean error of 5.21% on two multi-GPU platforms, our prediction pipeline generalizes well to other types of ML workloads, such as Transformer-based NLP models with a geomean error of 3.00%. Moreover, even without actually running ML workloads like DLRMs on the hardware, it is capable of generating insights such as quickly selecting the fastest embedding table sharding configuration (with a success rate of 85%).

==> tex/background.tex <==
\JDO{If the only subsection here is ``PyTorch training setups'', then make that the section title. This is really a methodology subsection, though, and should be presented as such. Do these design decisions/limitations apply to all pipelines you study? For the second two, it's not really clear to me what the tradeoff is, or if/how experts would quibble with these decisions. It would help if you explicitly said ``We take all our modeled pipelines directly from their source repos but we make the following changes before we model, and here are those changes and why we make them''.} \zhongyi{I was not sure about where to put it so I left it as a separate section here. I think it can come as the first subsection in Methodology, since in IV.B we are already talking about the benchmark and it's better to mention all the details before that. What do you think?} \JDO{It's fine to make it a separate section. But then maybe call the section ``Background: PyTorch Benchmark Setups'' (or I would just call it ``PyTorch Benchmark Setups''). I should add that I don't know \emph{anything} about PyTorch benchmark setups or even what they are so it's a mystery to me what this section is doing and to illuminate me here, I would need a couple of sentences here that describe the high level of setting up PyTorch and that any workloads run with PyTorch make a set of important decisions up front (?). I do think this section is a little less about ``configuring PyTorch'' and a little more about ``adapting existing benchmarks to our methodology/system''. The ``We take \ldots'' comment above IMHO still stands.} \zhongyi{I added some background here. I think Louis might be able to make it clearer if necessary. (Louis could you take a look at this?)} \JDO{I am comfortable with what's written here. But Louis needs to look at it, as you note.}

As our focus in this work is multi-GPU training of ML workloads, we describe the key configuration setups that we use to make our multi-GPU experiments run more efficiently and reliably with PyTorch.

\subsection{DistributedDataParallel (DDP) vs. DataParallel (DP)}
DDP and DP are two popular paradigms for distributed training with PyTorch. DDP's multi-process decentralized execution makes it a preferred choice for distributed training of ML models over DP for no GIL contention and less model replication and data movement overheads~\cite{Meta:2023:CBD}. \zhongyi{Louis: could you verify if what I'm saying is correct here?} \zhongyi{Done by replacing with performance-related argument.} Therefore, we focus on DDP (though with model parallelism for DLRM's embedding lookup module) throughout this work.

\subsection{Early Barrier}
\label{sec:early-barrier}
Conventionally there is no explicit barrier at the beginning of each batch in distributed training. Each rank reads its own mini-batch data independently, then kicks off the training of the batch, and only synchronizes at the first communication collective. However, it is common that for each batch the data ingestion latency is different across ranks, so the training on each rank might not start simultaneously and thus may incur a waiting time for other ranks when a communication collective is launched on some ranks. Since the profiler takes this time into account when it measures the collective time, it creates confusion in measurement and evaluation, especially when the loads such as embedding table shards in DLRMs on different ranks are imbalanced. Therefore, for evaluation and prediction purposes, we manually insert a barrier at the beginning of each batch to avoid this confusion and keep the latency of the first communication collective roughly equal across all ranks. This might introduce a random but tiny performance overhead compared to actual executions. However, ranks are synchronized at the end of training of the last batch by an \op{all-reduce}, and data ingestion is usually well-optimized (i.e., asynchronous and overlapped well by the training of the last batch) and not a bottleneck. Therefore, we can still expect our setup to be representative and accurately simulate the execution on a well-optimized training system with an almost simultaneous start on each rank.

\subsection{Gradient Bucketing}
Gradient bucketing~\cite{Li:PDE:2020} aims to resolve the problem of low bandwidth utilization and data-dependency-caused execution blocking due to frequent \op{all-reduce} launches and achieve higher throughput and lower latency. We adopt the default setting gradient bucket size (25~MB) in our experiments, as altering it only brings marginal benefits to the training performance for a very limited number of workloads. Notice that the execution trace of the first training iteration does \emph{not} reflect gradient bucketing because gradient exchange is completely unbucketed during the first iteration. We thus extract the execution traces of the second and onward iterations for prediction purposes.

